A Universal Trade-off Between the Model Size, Test Loss, and Training Loss of Linear Predictors

In this work we establish an algorithm and distribution independent non-asymptotic trade-off between the model size, excess test loss, and training loss of linear predictors. Specifically, we show that models that perform well on the test data (have low excess loss) are either "classical" -- have training loss close to the noise level, or are "modern" -- have a much larger number of parameters compared to the minimum needed to fit the training data exactly. We also provide a more precise asymptotic analysis when the limiting spectral distribution of the whitened features is Marchenko-Pastur. Remarkably, while the Marchenko-Pastur analysis is far more precise near the interpolation peak, where the number of parameters is just enough to fit the training data, it coincides exactly with the distribution independent bound as the level of overparametrization increases.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/general.tex <==
\section{Universal Lower Bound}\label{sec:main} 
First let us introduce some notation. We define the training data matrices 
\[
\Xtrain := \left(\bx_1^\sT, \ldots, \bx_n^\sT\right) \in \R^{n \times d},~~~~ \ytrain := (y_1, \ldots, y_n) \in \R^n
\]
so that $\data = (\Xtrain, \ytrain) \sim P^n$. If $(\bx, y) \sim P$ then we will use $P_X$ to denote the marginal distribution on $\bx$. We will use the following abbreviated notation for the expectations
\[
    \E_{\ytrain, \Xtrain} := \E_{\data \sim P^n},~~~~\E_{(\bx, y)} := \E_{(\bx, y) \sim P},~~~~\E_{\bx} := \E_{\bx \sim P_X}.
\]
We define the feature matrix and feature covariance matrix
\[
\bPhi := \left(\phi_p(\bx_1)^\sT, \ldots, \phi_p(\bx_n)^\sT\right) \in \R^{n \times p},~~~~ \bSigma := \E_{\bx}[\phi_p(\bx) \phi_p(\bx)^\sT] \in \R^{p \times p}.
\]
We will also make use of the whitened feature-matrix
\[
\bW := \bPhi \bSigma^{-1/2} \in \R^{n \times p}
\]
and the whitened empirical covariance matrix
\[
\bG := \frac{1}{p}\bW \bW^\sT \in \R^{p \times p}.
\]
We now state our main result
\begin{theorem}[Universal Lower Bound]\label{thm:general_lower_bound}
Let $n, p \geq 1$. Assume that $P$ and $\phi_p$ satisfy the following
\begin{enumerate}
    \item $\E y^2 < \infty$ which implies $\testloss(f_\star) < \infty$,\label{ass:integrable}
    \item $\Var(y \midsmall \bx) \geq \sigma^2$ almost surely over $\bx$,\label{ass:noise}
    \item $\rank(\bPhi) = \min(n, p)$ almost surely. \label{ass:rank}
\end{enumerate}
Then for any algorithm $\cA$ which outputs a linear feature model $\cA(\data)$ with training loss almost surely at most $\ofitlevel \sigma^2$
\[
\E_{\data \sim P^n}~ \excess(\cA(\data)) \geq \sigma^2 \frac{n}{p} (1 - \ofitlevel^{1/3})^4.
\]
\end{theorem}
\begin{remark}
Note that we can consider the feature map $\phi_p$ to be random as well, for instance taking $\phi_p$ to be a neural network with output dimension $p$ and random weights $\btheta$. It is often the case that Assumption~\ref{ass:rank} will hold almost surely over $\btheta$ (see Theorem~10 in \cite{holzmuller2020universality}). Since the weights are independent of the data, as an immediate corollary to Theorem \ref{thm:general_lower_bound} we get the same lower bound when additionally taking expectation over $\btheta$. 
\end{remark}
Under the assumptions of Theorem~\ref{thm:general_lower_bound} we define the minimal excess test loss of $\ofitlevel$-overfitting $p$-dimensional linear feature models trained on the dataset $\data$ of $n$ samples as
\[
    \minexcess(\ofitlevel; n, p) := \min_{\bbeta \in \R^p} \cE(\bbeta) \st \trainloss(\bbeta) \leq \ofitlevel \sigma^2.
\]
It then suffices to show that
\[
\E_{\data \sim P^n}[\minexcess(\ofitlevel; n, p)]\geq \sigma^2 \frac{n}{p} (1 - \ofitlevel^{1/3})^4.
\] 
We will bound the excess test loss $\excess(\bbeta)$ by comparing it with the excess loss with respect to the optimal linear model $\excess^{\lin}(\bbeta)$ which we characterize in the following three lemmas.
\begin{lemma}[Characterization of Optimal Linear Predictor]\label{lem:opt_lin}
Let $\bbeta_\star := \argmin_{\bbeta \in \R^p} R(\bbeta)$. Then 
\begin{enumerate}
    \item $\beta_\star$ is the orthogonal projection of $f_\star$ onto the subspace of linear functions $\cH = \{\beta(\bx) : \bbeta \in \R^p\}$ in $L^2$,\label{claim:opt_lin_proj}
    
    \item $\excess(f) := R(f) - R(f_\star) = \E_{\bx}[(f(\bx) - f_\star(\bx))^2$,\label{claim:excess}
    
    \item $\excess^{\lin}(\bbeta) := R(\bbeta) - R(\bbeta_\star) = \E_{\bx}[(\beta(\bx) - \beta_\star(\bx))^2]$.\label{claim:excess_lin}
\end{enumerate}
\end{lemma}
\begin{proof}
By definition of the optimal linear predictor
\begin{align*}
    \beta_\star &= \argmin_{\beta \in \cH} R(\beta)\\
    &= \argmin_{\beta \in \cH} \E_{(\bx, y)}[(y - \beta(\bx))^2]\\
     &= \argmin_{\beta \in \cH} \E_{(\bx, y)}[(y - f_\star(\bx))^2 + (f_\star(\bx) - \beta(\bx))^2] && (\text{since } \E_{y \mid \bx}[y - f_\star(\bx)] = 0)\\
     &= \argmin_{\beta \in \cH} \E_{\bx}[(f_\star(\bx) - \beta(\bx))^2],
\end{align*}
which shows Claim \ref{claim:opt_lin_proj}. For Claim \ref{claim:excess}
\begin{align*}
    R(f) - R(f_\star) &= \E_{(\bx, y)}[(y - f(\bx))^2] - \E_{(\bx, y)}[(y - f_\star(\bx))^2]\\
    &= \E_{(\bx, y)}[(f(\bx) - f_\star(\bx))^2] - 2\E_{(\bx, y)}[(f(\bx) - f_\star(\bx))(y - f_\star(\bx))]\\
    &= \E_{\bx}[(f(\bx) - f_\star(\bx))^2].
\end{align*}
% In the last equality we used the fact that since $f_\star(\bx) = \E(y \midsmall \bx)$
% \[
% \E_{y \mid \bx}[y - f_\star(\bx)] = 0.
% \]
For Claim \ref{claim:excess_lin}
\begin{align*}
    R(\bbeta) - R(\bbeta_\star) &= \excess(\bbeta) - \excess(\bbeta_\star)\\
    &=\E_{\bx} [(f_\star(\bx) - \beta(\bx))^2 - (f_\star(\bx) - \beta_{\star}(\bx))^2]\\
    &= \E_{\bx} [(\beta(\bx) - \beta_\star(\bx))^2] - 2\E_{\bx}[(f_\star(\bx) - \beta_{\star}(\bx))(\beta(\bx) - \beta_\star(\bx))]\\
    &= \E_{\bx} [(\beta(\bx) - \beta_\star(\bx))^2]
\end{align*}
where the second equality holds from Claim \ref{claim:excess} and the last equality holds from Claim \ref{claim:opt_lin_proj} in Lemma \ref{lem:opt_lin}.
\end{proof}
\begin{lemma}[Excess Linear Loss]\label{lem:excess_linear_loss}
The excess loss satisfies the following lower bound
\[
\excess(\bbeta) \geq \excess^{\lin}(\bbeta) = \norm{\bSigma^{1/2}(\bbeta - \bbeta_\star)}^2.
\]
\end{lemma}
\begin{proof}
It is clear that $\excess(\bbeta) \geq \excess^{\lin}(\bbeta)$. Using Lemma \ref{lem:opt_lin} and the definition of $\bSigma$
\begin{align*}
\excess(\bbeta) &= \E_{\bx}(\beta(\bx) - \beta_{\star}(\bx))^2 \\
&=\E_{\bx}(\bbeta^\sT \phi(\bx) - \bbeta_{\star}^\sT \phi(\bx))^2\\
&= (\bbeta - \bbeta_\star)^\sT \E_{\bx}[\phi(\bx)\phi(\bx)^\sT](\bbeta - \bbeta_\star)\\
&= \norm{\bSigma^{1/2}(\bbeta - \bbeta_\star)}^2.
\end{align*}
\end{proof}
\noindent Define the minimal excess linear loss $\auxmin(\ofitlevel)$ for training dataset $\data$ as
\[
\auxmin(\ofitlevel) = \min_{\bbeta \in \R^p} \excess^{\lin}(\bbeta) \st \trainloss(\bbeta) \leq \ofitlevel \sigma^2.
\]
Let $\bW = \bPhi \bSigma^{-1/2}$ be the whitened features. Define the random vectors
\[
\noise = (y_i - f_\star(\bx_i))_{i \in [n]} \in \R^n,~~~~ \linnoise = (f_\star(\bx_i) - \beta_\star(\bx_i))_{i \in [n]} \in \R^n
\]
and let $\effnoise = \noise + \linnoise$. We have the following characterization of the minimal excess linear loss.
\begin{lemma}[Minimal Excess Linear Loss]\label{lem:min_excess_risk_lower_bound}
We can equivalently write $\auxmin(\ofitlevel)$ as
\begin{equation}\label{eq:excess_linear_equiv}
    \min_{\boldb \in \R^p} \norm{\boldb}_2^2 \quad \mathrm{s.t.} \quad \frac{1}{n}\norm{\bW \boldb - \effnoise}_2^2 \leq \ofitlevel \sigma^2,
\end{equation}
and $\minexcess(\ofitlevel) \geq \auxmin(\ofitlevel)$.
\end{lemma}
\begin{proof}
By definition we can write the training loss as
\[
\trainloss(\bbeta) = \frac{1}{n} \norm{\bPhi \bbeta - \ytrain}^2.
\]
Note that $\ytrain = \bPhi \bbeta_\star + \effnoise$, hence
\begin{align*}
    \bPhi \bbeta - \ytrain &= \bPhi \bbeta - (\bPhi \bbeta_\star + \effnoise)\\
    &= \bPhi (\bbeta - \bbeta_\star) - \effnoise\\
    &= \bPhi \bSigma^{-1/2} \bSigma^{1/2} (\bbeta - \bbeta_\star) - \effnoise\\
    &= \bW \bSigma^{1/2} (\bbeta - \bbeta_\star) - \effnoise.
\end{align*}
Therefore by Lemma \ref{lem:excess_linear_loss} we see that $\auxmin(\ofitlevel)$ is equivalent to
\[
 \min_{\bbeta} \norm{\bSigma^{1/2}(\bbeta - \bbeta_\star)}^2 \st \frac{1}{n} \norm{\bW \bSigma^{1/2} (\bbeta - \bbeta_\star) - \effnoise}^2 \leq \ofitlevel \sigma^2
\]
which after making the following substitution over the optimization variable
\[
\boldb = \bSigma^{1/2}(\bbeta - \bbeta_\star)
\]
can be seen to be equivalent to Eq. (\ref{eq:excess_linear_equiv}). 
\end{proof}

\noindent We now proceed to lower bound $\auxmin(\ofitlevel)$ which will then imply the lower bound in Theorem \ref{thm:general_lower_bound} by the previous lemma. First we give a lemma that will be useful for dealing with the noise terms when obtaining the lower bound.
\begin{lemma}[Expectation Over Noise]\label{lem:expected_noise}
Let $f : \R^{n \times d} \to \S^n_+$ be any PSD matrix valued function. Then,
\begin{equation}\label{eq:expected_noise_lb}
    \E_{\ytrain, \Xtrain} [\effnoise^\sT f(\Xtrain) \effnoise] \geq \sigma^2 \E_{\Xtrain} \Tr(f(\Xtrain)).
\end{equation}
Moreover, if $\Var(y \midsmall \bx) = \sigma^2$ almost surely and $f_\star = \beta_\star$ then the above is an equality.
\end{lemma}
\begin{proof}
Recalling that $\effnoise = \noise + \linnoise$. By definition of $\noise$ we have that
\[
\E_{\ytrain \mid \Xtrain}[\noise] = \bzero
\]
and by the assumption on the noise variance we have almost surely
\begin{equation}\label{eq:noise_covariance}
    \E_{\ytrain \mid \Xtrain}[\noise \noise^\sT] = \diag((\Var[y \mid \bx_i])_{i \in [n]}) \succeq \sigma^2 \id.
\end{equation}
Using these observations we have 
\begin{align*}
    \E_{\ytrain \mid \Xtrain} [\effnoise^\sT f(\Xtrain) \effnoise] &= \E_{\ytrain \mid \Xtrain} [\noise^\sT f(\Xtrain) \noise] + 2\E_{\ytrain \mid \Xtrain} [\linnoise^\sT f(\Xtrain) \noise] + \E_{\ytrain \mid \Xtrain} [\linnoise^\sT f(\Xtrain) \linnoise]\\
    &= \Tr(f(\Xtrain) \E_{\ytrain \mid \Xtrain} [\noise \noise^\sT]) + 2 \linnoise^\sT f(\Xtrain) \E_{\ytrain \mid \Xtrain}[\noise] + \linnoise^\sT f(\Xtrain) \linnoise\\
    &= \Tr(f(\Xtrain) \E_{\ytrain \mid \Xtrain} [\noise \noise^\sT]) + \linnoise^\sT f(\Xtrain) \linnoise \\
    &\geq \sigma^2 \Tr(f(\Xtrain)) + \linnoise^\sT f(\Xtrain) \linnoise \\
    &\geq \sigma^2 \Tr(f(\Xtrain)),
\end{align*}
where we used Eq.  (\ref{eq:noise_covariance}) in the first inequality and we used the assumption that $f(\bX)$ is a PSD matrix for the last inequality.
By iterating expectations we have
\[
\E_{\ytrain,\Xtrain} [\effnoise^\sT f(\Xtrain) \effnoise] = \E_{\Xtrain} \E_{\ytrain \mid \Xtrain} [\effnoise^\sT f(\Xtrain) \effnoise] \geq \sigma^2 \E_{\Xtrain} \Tr(f(\Xtrain))
\]
as desired. Note that if $\Var(y \midsmall \bx) = \sigma^2$ then Eq.  (\ref{eq:noise_covariance}) becomes an equality and if $f_\star = \beta_\star$ then $\linnoise = \bzero$ and so it easy to see that Eq.  (\ref{eq:expected_noise_lb}) is an equality as well.
\end{proof}
\begin{proof}[Proof of Theorem \ref{thm:general_lower_bound}]
Consider the optimization problem defining $\auxmin(\ofitlevel)$. The associated Lagrangian is
\[
    \cL(\boldb, \lmult) = \norm{\boldb}_2^2 + \lmult\qty(\frac{1}{n} \norm{\bW \boldb - \effnoise}_2^2 - \ofitlevel \sigma^2)
\]
for $\lmult \geq 0$ and the dual function is
\[
g(\lmult) = \inf_{\boldb} \cL(\boldb, \lmult).
\]
After some rearrangement, we can rewrite the Lagrangian as
\[
\cL(\boldb, \lmult) = \boldb^\sT\qty(\id + \frac{\lmult}{n} \bW^\sT \bW)\boldb - \frac{2 \lmult}{n} \boldb^\sT \bW \effnoise + \frac{\lmult}{n}\norm{\effnoise}_2^2 - 
\lmult \ofitlevel \sigma^2
\]
which is easily seen to be a convex quadratic objective in $\boldb$, hence we can minimize by setting the derivative to zero. The gradient is given by 
\begin{align*}
    \grad_{\boldb} \cL(\boldb, \lmult) &= 2\qty(\id + \frac{\lmult}{n} \bW^\sT \bW) \boldb - \frac{2 \lmult}{n} \bW^\sT \effnoise
\end{align*}
hence setting this equal to zero and solving for the optimal $\boldb$ we get
\begin{align*}
    \boldb_\star(\lmult) &= \argmin_{\boldb} \cL(\boldb, \lmult)\\
    &= \lmult(n\id + \lmult \bW^\sT \bW)^{-1}\bW^\sT \effnoise\\
    &= \bW^\sT((n/\lmult)\id + \bW \bW^\sT)^{-1}\effnoise\\
    &= \frac{1}{p}\bW^\sT\qty(\frac{n}{p} \frac{1}{\lmult}\id + \frac{1}{p} \bW \bW^\sT)^{-1}\effnoise.
\end{align*}
By weak duality we have that for any $\lmult \geq 0$,
\[
    \auxmin(\ofitlevel) \geq g(\lmult) = \cL(\boldb_\star(\lmult), \lmult).
\]
For convenience we make the following change of variables 
\[
\ridgeparam := \frac{n}{p} \frac{1}{\lmult}
\]
which is a bijection between $[0, +\infty]$ and itself. Thus in terms of $\ridgeparam$ we can write
\begin{align*}
    \cL(\boldb, \ridgeparam) &= \norm{\boldb}^2 + \frac{n}{p\ridgeparam} \qty(\frac{1}{n}\norm{\bW \boldb - \effnoise}^2 - \ofitlevel \sigma^2)\\
    \boldb_\star(\ridgeparam) &= \bW^\sT(\ridgeparam \id + \bW \bW^\sT)^{-1} \effnoise
\end{align*}
and for all $\ridgeparam \geq 0$ we have the lower bound
\[
\auxmin(\ofitlevel) \geq g(\ridgeparam).
\]
Taking expectations, we have the following bound
\begin{equation}\label{eq:expected_dual}
    \E_{\ytrain, \Xtrain} \auxmin(\ofitlevel) \geq \E_{\ytrain, \Xtrain} \cL(\boldb_\star(\ridgeparam), \ridgeparam) = \E_{\ytrain, \Xtrain} \norm{\boldb_\star(\ridgeparam)}^2 + \frac{n}{p \ridgeparam} \E_{\ytrain, \Xtrain} \qty(\frac{1}{n}\norm{\bW \boldb_\star(\ridgeparam) - \effnoise}_2^2 - \ofitlevel \sigma^2).
\end{equation}
Let $\bG = \bW\bW^{\sT}/p$ and $\bG(\ridgeparam) = \bG + \ridgeparam \id$. Denote the eigenvalues of $\bG$ as $\lambda_1 \geq \lambda_2 \geq \ldots \geq \lambda_n$. We will show
\begin{align}
    \E_{\ytrain, \Xtrain} \norm{\boldb_\star(\ridgeparam)}^2 \geq \frac{\sigma^2}{p} \E_{\Xtrain} \Tr(\bG(\ridgeparam)^{-1} \bG \bG(\ridgeparam)^{-1}) &= \frac{\sigma^2}{p} \E_{\Xtrain} \sum\limits_{i = 1}^n \frac{\lambda_i}{(\lambda_i + \ridgeparam)^2} \label{eq:expected-norm}\\
    \E_{\ytrain, \Xtrain} \frac{1}{n}\norm{\bW \boldb_\star(\ridgeparam) - \effnoise}_2^2 \geq \frac{\sigma^2}{n} \E_{\Xtrain} \Tr(\bG \bG(\ridgeparam)^{-1} - \id)^2 &= \frac{\sigma^2}{n} \E_{\Xtrain} \sum\limits_{i = 1}^n \qty(\frac{\ridgeparam}{\lambda_i + \ridgeparam})^2 \label{eq:expected-constraint}
\end{align}
using Lemma \ref{lem:expected_noise}. For Eq. (\ref{eq:expected-norm}) we have the following
\begin{align*}
    \E_{\ytrain, \Xtrain} \norm{\boldb_\star(\ridgeparam)}^2 &= \frac{1}{p} \E_{\ytrain, \Xtrain} \effnoise^\sT \bG(\ridgeparam)^{-1} \bG \bG(\ridgeparam)^{-1} \effnoise\\
    &\geq \frac{\sigma^2}{p} \E_{\Xtrain} \Tr(\bG(\ridgeparam)^{-1} \bG \bG(\ridgeparam)^{-1}).
\end{align*}
Similarly, for Eq. (\ref{eq:expected-constraint})
\begin{align*}
    \E_{\ytrain, \Xtrain} \frac{1}{n}\norm{\bW \boldb_\star(\ridgeparam) - \effnoise}_2^2 &= \frac{1}{n}\E_{\ytrain, \Xtrain} [\effnoise^\sT(\bG \bG(\ridgeparam)^{-1} - \id)^2\effnoise] \\
    &\geq \frac{\sigma^2}{n} \E_{\Xtrain} \Tr(\bG \bG(\ridgeparam)^{-1} - \id)^2.
\end{align*}
Note that by the full rank assumption, $\lambda_1 \geq \cdots \geq \lambda_{\min(n, p)} > 0$ and $\lambda_{\min(n, p) + 1} = \ldots = \lambda_n = 0$ almost surely. Define the function $f : [0, +\infty] \to \R$ as
\[
f(\ridgeparam) := \frac{1}{n}\sum\limits_{i = 1}^n \qty(\frac{\ridgeparam}{\lambda_i + \ridgeparam})^2 = \frac{1}{n}\sum\limits_{i = 1}^{\min(n, p)} \qty(\frac{\ridgeparam }{ \lambda_i + \ridgeparam })^2 + \max(0, 1 - p/n).
\]
Note that $f$ is continuous and $\inf_\ridgeparam f(\ridgeparam) = f(0) = \max(0, 1 - p/n)$ and $\sup_\ridgeparam f(\ridgeparam) = f(\infty) = 1$. Therefore as long as $1 - p/n \leq \ofitlevel$ there exists $\ridgeparam_\star$ such that 
\begin{equation}\label{eq:lagrange_multiplier_fixed_point}
    f(\ridgeparam_\star) = \frac{1}{n} \sum\limits_{i = 1}^n \qty(\frac{\ridgeparam_\star}{\lambda_i + \ridgeparam_\star})^2 = \ofitlevel.
\end{equation}
Otherwise if $p/n \geq 1 - \ofitlevel$, then by taking $\ridgeparam \to 0$, we have that 
\[
   \frac{1}{\ridgeparam} \cdot \E_{\ytrain, \Xtrain} (\norm{\bW \boldb_\star(\ridgeparam) - \effnoise}_2^2 - \ofitlevel \sigma^2) \to \infty,
\]
which by inequality Eq. (\ref{eq:expected_dual}) implies $\E_{\ytrain, \Xtrain} ~\auxmin(\ofitlevel) = +\infty$ and any lower bound holds trivially. Thus we will assume that $p/n \leq 1 - \ofitlevel$. Let $\ridgeparam_\star$ be the random variable dependent on $\Xtrain$ that satisfies Eq. (\ref{eq:lagrange_multiplier_fixed_point}). Then by Eq. (\ref{eq:expected-constraint}) we have that
\[
\frac{1}{n}\norm{\bW \boldb_\star(\ridgeparam_\star) - \effnoise}_2^2 - \ofitlevel \sigma^2 \geq 0.
\]
Thus we have that
\begin{equation}\label{eq:excess-lb-opt-lagrange}
    \E_{\ytrain, \Xtrain} \auxmin(\ofitlevel)  \geq \frac{\sigma^2}{p} \E_{\Xtrain} \sum\limits_{i = 1}^n \frac{\lambda_i}{(\lambda_i + \ridgeparam_\star)^2},
\end{equation}
since from Eq. (\ref{eq:expected_dual})
\begin{align*}
    \E_{\ytrain, \Xtrain} \auxmin(\ofitlevel) &\geq \E_{\ytrain, \Xtrain} \norm{\boldb_\star(\ridgeparam_\star)}^2 + \frac{n}{p \ridgeparam_\star} \E_{\ytrain, \Xtrain} \qty(\frac{1}{n}\norm{\bW \boldb_\star(\ridgeparam_\star) - \effnoise}_2^2 - \ofitlevel \sigma^2)\\
    &\geq \E_{\ytrain, \Xtrain} \norm{\boldb_\star(\ridgeparam_\star)}^2\\
    &\geq \frac{\sigma^2}{p} \E_{\Xtrain} \sum\limits_{i = 1}^n \frac{\lambda_i}{(\lambda_i + \ridgeparam_\star)^2},
\end{align*}
where the last inequality is Eq. (\ref{eq:expected-norm}). Observe that from Eq. (\ref{eq:asymp_fixed_point})
\[
    \tau = \frac{1}{n} \sum\limits_{i = 1}^n \qty(\frac{\ridgeparam_\star}{\lambda_i + \ridgeparam_\star})^2 
    \leq \frac{1}{n} \sum\limits_{i = 1}^n \qty(\frac{\ridgeparam_\star}{\lambda_n + \ridgeparam_\star})^2
    =\qty(\frac{\ridgeparam_\star}{\lambda_n + \ridgeparam_\star})^2
\]
which implies that 
\begin{equation}\label{eq:multiplier_value_lower_bound}
    \ridgeparam_\star \geq \frac{\ofitlevel^{1/2}}{1 - \ofitlevel^{1/2}} \cdot \lambda_n.
\end{equation}
Define the constant 
\[
    \delta_0 = \frac{\ofitlevel^{1/2}}{1 - \ofitlevel^{1/2}},
\]
and take some constant $\delta \geq \delta_0$ which will be chosen later. Let $m(\delta) \in \{0, 1, \ldots, n-1\}$ be defined so that
\begin{equation}\label{eq:eigval_multiplier_spacing}
    \delta \lambda_{m(\delta)} > \ridgeparam_\star \geq \delta \lambda_{m(\delta)+1},
\end{equation}
where we define $\lambda_0 = +\infty$. Note that from Eq. (\ref{eq:multiplier_value_lower_bound}) and our choice of $\delta_0$ that $m(\delta)$ is well-defined. Observe that 
\begin{align*}
    \ofitlevel &\geq \frac{1}{n}\sum\limits_{i = m(\delta) + 1}^n \qty(\frac{\ridgeparam_{\star}}{\lambda_i + \ridgeparam_{\star}})^2\\
    &\geq \frac{1}{n} \sum\limits_{i = m(\delta) + 1}^n \frac{1}{(\delta^{-1} + 1)^2} = \frac{1}{n} \frac{n - m(\delta)}{(1 + \delta^{-1})^2}
\end{align*}
which after rearranging implies that
\begin{equation}\label{eq:m_delta_lower_bound}
    m(\delta) \geq n\qty[1 - \ofitlevel(1 + \delta^{-1})^2].
\end{equation}
Therefore from Eq. (\ref{eq:excess-lb-opt-lagrange}), we have that 
\begin{align*}
    \E_{\ytrain, \Xtrain} \auxmin(\ofitlevel) &\geq \frac{\sigma^2}{p} \E_{\Xtrain} \sum\limits_{i = 1}^n \frac{\lambda_i}{(\lambda_i + \ridgeparam_\star)^2}\\
    &\geq \frac{\sigma^2}{p(1 + \delta)^2 } \E_{\Xtrain} \sum\limits_{i = 1}^{m(\delta)} \frac{1}{\lambda_i} && \text{(by Eq. (\ref{eq:eigval_multiplier_spacing}))}\\
    &\geq \frac{\sigma^2}{p(1 + \delta)^2 } \E_{\Xtrain} m(\delta)^2 \cdot \qty(\sum\limits_{i = 1}^{m(\delta)} \lambda_i)^{-1} && \text{(by AM-HM ineq. Lemma \ref{lem:AM-HM})}\\
    &\geq \frac{\sigma^2 n^2 \qty[1 - \ofitlevel(1 + \delta^{-1})^2]^2}{p(1 + \delta)^2 } \E_{\Xtrain} \qty(\sum\limits_{i = 1}^{m(\delta)} \lambda_i)^{-1}\\
    &\geq \frac{\sigma^2 n^2 \qty[1 - \ofitlevel(1 + \delta^{-1})^2]^2}{p(1 + \delta)^2 } \qty(\E_{\Xtrain} \sum\limits_{i = 1}^{n} \lambda_i)^{-1} && \text{(by Jensen's Inequality)}\\
    &= \frac{\sigma^2  n^2 \qty[1 - \ofitlevel(1 + \delta^{-1})^2]^2}{p(1 + \delta)^2} \cdot \frac{1}{n} \\
    &= \frac{\sigma^2 [1 - \ofitlevel(1 + \delta^{-1})^2]^2}{(1 + \delta)^2 } \frac{n}{p}.
\end{align*}
Recall that $\delta_0 = \frac{\ofitlevel^{1/2}}{1 - \ofitlevel^{1/2}}$. By taking $\delta = \frac{\ofitlevel^{1/3}}{1 - \ofitlevel^{1/3}} \geq \delta_0$ we see that 
\[
\frac{[1 - \ofitlevel(1 + \delta^{-1})^2]^2}{(1 + \delta)^2 } = (1 - \ofitlevel^{1/3})^4,
\]
hence for this choice of $\delta$
\[
    \E_{\ytrain, \Xtrain} \auxmin(\ofitlevel) \geq \frac{\sigma^2 [1 - \ofitlevel(1 + \delta^{-1})^2]^2}{(1 + \delta)^2 } \frac{n}{p} = \sigma^2 \frac{n}{p}(1 - \ofitlevel^{1/3})^4.
\]
Since $\minexcess(\ofitlevel) \geq \auxmin(\ofitlevel)$, taking expectations over the data and using the above inequality shows the desired claim.
\end{proof}

==> sections/setting.tex <==
\section{Setting and Notation}
We consider general regression problems where we are given a training set of $n$ samples $\{(\bx_i, y_i)\}_{i=1}^n$ with $\bx_i \in \R^d$ and $y_i \in \R$. Each sample $(\bx_i, y_i) \simiid P$ for some distribution $P$ on $\R^d \times \R$. We define 
\[
\Xtrain := \left(\bx_1^\sT, \ldots, \bx_n^\sT\right) \in \R^{n \times d},~~~~ \ytrain := (y_1, \ldots, y_n) \in \R^n.
\]
Let $(\bx, y) \sim P$ be a new sample independent of the training set. We will denote by $P_X$ the marginal distribution of $\bx$. For a function $f: \R^d \to \R$ we define its train loss $\trainloss(f)$ and its test loss $\testloss(f)$ as
\[
    \trainloss(f) := \frac{1}{n} \sum\limits_{i=1}^n (y - f(\bx_i))^2,~~~~ \testloss(f) := \E_{(\bx, y)}(y - f(\bx))^2.
\]
Note that if we define $f_\star(\bx)$ to the the conditional expectation $\E(y \mid \bx)$ then $f_\star$ minimizes $R(f)$ and we can write the excess test loss as
\[
\cE(f) := \testloss(f) - \testloss(f_\star) = \E_{(\bx, y)}(f_\star(\bx) - f(\bx))^2.
\]
Given a $p$-dimensional feature map $\phi_p: \R^d \to \R^p$ we will consider linear feature models $f_{\bbeta}$ of the form
\[
    f_{\bbeta}(\bx) = \bbeta^\sT \phi_p(\bx)
\]
for some $\bbeta \in \R^p$ and will identify $\bbeta$ with $f_\bbeta$ for example when writing $\cE(\bbeta)$ in place of $\cE(f_\bbeta)$. We will also define
\[
\bPhi := \left(\phi_p(\bx_1)^\sT, \ldots, \phi_p(\bx_n)^\sT\right) \in \R^{n \times p}.
\]
Define the covariance matrix
\[
\bSigma := \E_{\bx}[\phi_p(\bx) \phi_p(\bx)^\sT] \in \R^{p \times p}.
\]
